Reduced basis stabilization and post-processing for the virtual element method

We present a reduced basis method for cheaply constructing (possibly rough) approximations to the nodal basis functions of the virtual element space, and propose to use such approximations for the design of the stabilization term in the virtual element method and for the post-processing of the solution.

==> test0.tex <==
% ==============================================
\section{Application I: Stabilization}\label{sec:stab}

As mentioned in Section \ref{sec:intro}, we can exploit the possibility of cheaply constructing approximations to the basis functions of the local virtual element space, to design of ad hoc local stabilization bilinear forms for strongly anisotropic problems. 




The idea is to define $\shloc$ as
\[
\shloc(
e_i,e_j
) = \haloc(\widehat e_{M,i}^{\,\text{rb}}[K],\widehat e_{M,j}^{\,\text{rb}}[K]), 
\]
where
\[
\haloc(u,w) = \sum_{i=1}^{N} \int_{\That_i} \rosso{| \det(\Bmatr^{-1}_{\elementVEM,i})|}\, \Bmatr_{\elementVEM,i}^\top\, \aa\, \Bmatr_{\elementVEM,i}\grad\widehat{u}\cdot\grad\widehat{v}\,d\xhat
\]
is the bilinear form on the reference element obtained by change of variable from the bilinear form~$\aloc$. 


As far as the choice of the size $M$ of the reduced basis is concerned, we observe that 
taking a large value of $M$ would ideally result in accurately reconstructing the local shape functions and, consequently, in taking $\shloc \sim \aloc$. In other words, for $M$ large, rather than a virtual element method we would have a polygonal finite element method, based on the virtual elements discrete space, which, in the lowest order case considered here, coincides with the polygonal finite element space with harmonic barycentric coordinates \cite{martin2008polyhedral,DeRose2006HarmonicC}. 
In the spirit of the virtual element method, we rather take $M$ small/very small, so that $\shloc$ only roughly approximates $\aloc$. 
We observe that $\shloc(
e_i,e_j
)$ can be computed efficiently thanks to the affine decomposition. Indeed, we have
\begin{equation}
	\shloc(
	e_i,e_j
	)  =
	\haloc(  \hTheta_i, 
	\hTheta_j 
	) + \sum_{\ell=1}^M w^{K,i}_\ell
	\haloc(   \xiHat_i^\ell, 
	\hTheta_j
	) +  \sum_{\ell=1}^M \wljK
	\haloc(  \hTheta_i , 
	\xiHat_j^\ell
	)
	+  \sum_{\ell,\ell'=1}^M 
	\wljK
	\haloc(  \xiHat_i^{\ell'}, 
	\xiHat_j^\ell
	),\label{affinestab}
\end{equation}
where $\wljK$ are the coefficient in the expansion \eqref{rbsolution}.
\blu{As we already did in \eqref{eq:matr_dec},} the matrix 
$\rosso{| \det(\Bmatr^{-1}_{\elementVEM,i})|}\, \Bmatr_{\elementVEM,i}^\top\, \Kmatr\, \Bmatr_{\elementVEM,i}
$ can be easily decomposed as 
\[
\rosso{| \det(\Bmatr^{-1}_{\elementVEM,i})|}\, \Bmatr_{\elementVEM,i}^\top\, \aa\, \Bmatr_{\elementVEM,i} = \sum_{\nu = 1}^4 \coef_\nu^i[K] \Acal^\nu,
\]
where, for $\nu = 1,2,3$, $\Acal^\nu$ is defined in \eqref{def:symmatbasis} and 
\[
\Acal^4= \begin{bmatrix}
	0 & 1 \\
	-1 & 0
\end{bmatrix},
\]
so that we have
\[
\haloc(\xiHat_{j}^\ell,\xiHat_{j^\prime}^{\ell'}) = \sum_{i=1}^N \sum_{\nu = 1}^4 \coef_\nu^i[K] \Amatr_i^\nu(j,{j^\prime},\ell,\ell'). 
\]
Then, having precomputed $\Amatr^{\nu}_i$, $i=1,\cdots,N$, $\nu = 1,\cdots,4$, the right hand side of \eqref{affinestab} is easily  assembled. 








\input{algorithm_rbstab}

\rev{ The proposed stabilization is of course more expensive than standard diagonal stabilizations such as \emph{dofi-dofi} or \emph{D-recipe}. For the reduced basis stabilization, the bulk of the computational cost of the construction of $S^ K_h$ lies in the evaluation of the coefficients $\wljK$, for which we refer to Table \ref{tab:times1}. Its overall cost is of the same order of magnitude of the cost of the evaluation of the consistency component of the stiffness matrix. Conversely, standard diagonal stabilization terms such as \emph{dofi-dofi} or \emph{D-recipe} are  extremely cheap, their cost being two to three orders of magnitude lower, and therefore, overall negligible. On the other hand, as we will see below, depending on the problem, the reduced basis stabilization might lead to an improvement in the convergence of the method that, in our opinion, makes such computational overhead acceptable. }

\

\rev{
	%We observe that the condition number of the stiffness matrix computed with the RB stabilization is comparable with the condition number of both the matrix assembled with \emph{dofi--dofi} stabilization and the ``true'' stiffness, computed by explicitly solving the PDE associated to each virtual basis function. This fact is depicted in Figure~\ref{fig:cond}, where we plot the behavior of the condition numbers for the Poisson equation on Voronoi meshes.
	%We observe that the condition number of the stiffness matrix computed with the RB stabilization is comparable with the condition number of the matrices assembled with \emph{dofi--dofi} stabilization and by explicitly solving the PDE associated to each virtual basis function (``true'' stiffness). This fact is depicted in Figure~\ref{fig:cond}, where we plot the behavior of the condition numbers for the Poisson equation on Voronoi meshes.
	%The condition number of the stiffness matrix obtained through RB stabilization exhibits the same behavior of the condition numbers of matrices assembled using the \textit{dofi--dofi} stabilization and by explicitly solving the PDE associated with each virtual basis function (``true'' stiffness). This fact is depicted in Figure~\ref{fig:cond}, where we plot the behavior of the condition numbers for the Poisson equation on Voronoi meshes.
	
	To assess the performance of the new reduced basis  stabilization, we start by comparing the condition number of the resulting stiffness matrix with the condition number of, on the one hand, the standard VEM stiffness matrix with  \emph{dofi--dofi} and \emph{D-recipe} stabilizations, and, on the other hand, the ideal (non computable) stiffness matrix, which we assembled after constructing the virtual basis functions by means of a finite element solution of the local PDE \eqref{truebasisfunctions}.   
	On a unit squared domain, we consider both a Laplace operator, and two anisotropic diffusion problems with diffusivity tensors $\aa_1$ and $\aa_2$ respectively defined as
	\[
	\aa_1 = \begin{bmatrix}
		1 & 10^{-2} \\
		5\cdot10^{-3} & 10^{-4}
	\end{bmatrix}, \qquad \qquad \aa_2 = \begin{bmatrix}
		1 & 10^{-2} \\
		5\cdot10^{-3} & 10^{-4}
	\end{bmatrix}.
	\]
	
	These are the diffusivity tensors that we will later use for the convergence tests. In Figure~\ref{fig:cond},  we plot the evolution of the condition numbers for the different operators discretized on a sequence of Voronoi meshes generated by means of Polymesher~\cite{polymesher}  (see, for instance, Figure~\ref{fig:mesh_voro}). We observe that 
	the condition number of the stiffness matrix obtained through RB stabilization exhibits the same behavior of the condition numbers of both the standard VEM matrix
	and the ``true'' stiffness. 
	
	
	\begin{figure}%[h!]
		\centering
		\textbf{Condition number}
		\subfloat{\includegraphics[width=0.34\linewidth]{figures/cond_poisson}}
		\subfloat{\includegraphics[width=0.34\linewidth]{figures/cond_test1}}
		\subfloat{\includegraphics[width=0.34\linewidth]{figures/cond_test2}}
		%\caption{\rev{Condition number of the stiffness matrix arising from the discretization of the Poisson equation on Voronoi meshes. The blue line refers to the standard VEM matrix constructed with \textit{dofi--dofi} stabilization, whereas the red line represents the condition number of the ``true'' stiffness, constructed by explicitly computing the virtual basis functions. Finally, the green line and the black circles refers to the RB stabilization case, with $M=1,\,60$ respectively. The methods exhibit the same behavior.}}
		% It is clear that the results of all the considered techniques are comparable.
		\caption{\rev{From left to right: behavior of the condition number for the Poisson problem, Test~1 ($\aa = \aa_1$) and Test~2 ($\aa=\aa_2$). In the three cases we observe no significant difference between the different versions of the VEM method.}}
		\label{fig:cond}
	\end{figure}
	
	
}


\

\rev{
	Focusing on strongly anisotropic problems, where the standard lowest order VEM formulations have been observed to show poor performance \rosso{(see \cite{berrone2022comparison})}, we next compare the convergence properties of the  reduced basis stabilization,  with  the \textit{dofi--dofi} and \textit{D--recipe}, on three test cases. 
	For all the cases, we consider Problem~\ref{pro:cont_poisson} with strongly anisotropic solutions and diffusivity tensors. The domain $\Omega$ is once again the unit square, discretized by a sequence of Voronoi meshes generated by means of Polymesher~\cite{polymesher}. }
\begin{figure}%[h!]
	\centering
	\includegraphics[width=0.325\linewidth]{figures/mesh256}
	\includegraphics[width=0.32\linewidth]{figures/mesh512}
	\includegraphics[width=0.32\linewidth]{figures/mesh1024}
	\caption{Example of Voronoi meshes for the unit square.}
	\label{fig:mesh_voro}
\end{figure}
In order to evaluate the performance of the methods, we introduce the following two relative error norms: for $\diamond = u^\text{fe}_h, \PiNabla u_h,\uhRB$ and $\Square = u^\text{fe}_h, \uhRB$, we set
\begin{equation*}
	\begin{aligned}
		&\errstar{\diamond} = \frac{ \bigg( \sum_{\elementVEM\in\mesh} \norm{u-\diamond}^2_{\star,\elementVEM}\bigg)^{\frac12} }{\norm{u}_{\star,\Omega}}&\quad\text{ for }\quad\star=0,1\\
		&\erren{\diamond} = \frac{ \bigg( \sum_{\elementVEM\in\mesh} \norm{ \sqrt{\Kmatr} \grad \big( u-\diamond \big)}^2_{0,\elementVEM}\bigg)^{\frac12} }{\norm{\sqrt{\Kmatr}\grad u}_{0,\Omega}}&\\
		&\errinf{\Square} = \frac{\max_{\x\in\Omega}|u-\Square|}{\max_{\x\in\Omega}|u|}&
	\end{aligned}
\end{equation*}	
As customary for the virtual element method, for the tests in this section, we evaluate $\errstar{\diamond}$ and $\erren{\diamond}$ with  $\diamond = \PiNabla u_h$ (that is, we do not reconstruct the full discrete solution by either the RB method or the finite element method).




\subsubsection*{Test 1.}  For this test, we choose the right hand side so that the following exact solution is obtained %\rosso{[Test 2 della cartella dei risultati]}
\begin{equation}\label{eq:sol_test_1}
	u(x,y) = \sin(2\pi x)\sin(\parr\pi y),\qquad \parr=80.
\end{equation}
The solution is characterized by high frequency oscillations in $y$ direction. We set the diffusivity tensor to be $\aa = \aa_1$.
A simplified plot of the exact solution $u$ when $\parr=10$ in reported in Figure~\ref{fig:exact_u_1}. Convergence plots for this test are collected in Figure~\ref{fig:stab_test_1}, while the convergence history is reported in Table~\ref{tab:errors_test1} for the case of \textit{dofi--dofi} stabilization and RB stabilization built considering $M=1$. We notice that the reduced basis stabilization improves the convergence properties of the method for both $\erruno{\PiNabla u_h}$ and $\erren{\PiNabla u_h}$, with respect to the use of \textit{dofi--dofi} and \textit{D--recipe} (which, in this case, produce equivalent results). This improvement can already be observed  when just one reduced basis function is considered ($M=1$). Moreover, we notice that by increasing the number of reduced bases involved in the stabilization (we consider, in  particular, $M=10,60$), we do not obtain a significant gain with respect to $M=1$, which is then sufficient to cheaply take into account the anisotropy of the problem.

\begin{figure}%[h!]
	\centering
	\includegraphics[width=0.45\linewidth]{figures/stabilization/test1_plot}\quad
	\includegraphics[width=0.45\linewidth]{figures/stabilization/test1_cont}
	\caption{Surface plot and contour plot for the exact solution $u$ defined in \eqref{eq:sol_test_1}. In this case, we set $\parr=10$.}
	\label{fig:exact_u_1}
\end{figure}

\begin{figure}%[h!]
	\centering
	\textbf{Comparison of stabilization terms - Test 1}
	\subfloat{\includegraphics[width=0.43\linewidth]{figures/stabilization/test_1_h1}}
	\subfloat{\includegraphics[width=0.43\linewidth]{figures/stabilization/test_1_en}}
	\caption{Convergence plots for Test 1. From left to right, $\erruno{\PiNabla u_h}$ and $\erren{\PiNabla u_h}$. We denote in blue the convergence for \textit{dofi--dofi}, while yellow is used for \textit{D--recipe}. For the reduced basis stabilization, we denote in green the case $M=1$, in red $M=10$ and with black circles $M=60$. In both plots, it is evident that the reduced basis stabilization performs better than the standard choices because it is able to catch the anisotropy of the problem. \rosso{The proposed RB method is effective in the cheapest case since $M=1,10,60$ provide equivalent results.}}%Since $M=1,10,60$ show the same behavior, using just one basis we are able to take into account the entire information given by the reduced basis.}
\label{fig:stab_test_1}
\end{figure}

\renewcommand{\arraystretch}{1.4}
\begin{table}
\begin{center}
	\begin{tabular}{c||rr|rr||rr|rr}
		%\hline
		\multicolumn{9}{c}{\textbf{Test 1 - Convergence history}}\\
		\hline
		& \multicolumn{4}{c||}{\em dofi--dofi} & \multicolumn{4}{c}{Reduced Basis, $M=1$} \\
		\hline
		$h$ & $\erruno{\PiNabla u_h}$ & Rate & $\erren{\PiNabla u_h}$ & Rate & $\erruno{\PiNabla u_h}$ & Rate & $\erren{\PiNabla u_h}$ & Rate  \\
		\hline
		3.021e-2	& 9.971e-1	& --	& 9.989e-1	& --	& 9.945e-1	& --	& 9.966e-1	& --   \\
		1.536e-2	& 9.822e-1	& 0.02	& 9.841e-1	& 0.02	& 9.643e-1	& 0.05	& 9.671e-1	& 0.04 \\
		7.569e-3	& 9.269e-1	& 0.08	& 9.304e-1	& 0.08	& 8.586e-1	& 0.16	& 8.641e-1	& 0.16 \\
		5.548e-3	& 8.625e-1	& 0.23	& 8.683e-1	& 0.22	& 7.498e-1	& 0.44	& 7.583e-1	& 0.42 \\
		4.094e-3	& 7.561e-1	& 0.43	& 7.659e-1	& 0.41	& 5.968e-1	& 0.75	& 6.095e-1	& 0.72 \\
		3.219e-3	& 6.088e-1	& 0.90	& 6.239e-1	& 0.85	& 4.264e-1	& 1.40	& 4.436e-1	& 1.32 \\
		2.063e-3	& 4.365e-1	& 0.74	& 4.578e-1	& 0.70	& 2.709e-1	& 1.02	& 2.919e-1	& 0.94 \\
		\hline
	\end{tabular}
\end{center}
\caption{Errors and convergence rates for Test 1. We focus on VEM with \emph{dofi--dofi} stabilization and reduced basis stabilization with $M=1$.}
\label{tab:errors_test1}
\end{table}
\renewcommand{\arraystretch}{1}
%

\rev{
\subsubsection*{Test 2.} For this test, the right hand side is computed in such a way that the exact solution for the considered problem is the following function, which is singular when $x=0$,
\begin{equation}\label{eq:sol_test_3}
	u(x,y) = \sin(2\pi x)\sin(\parr\pi y)\log(x),\qquad \parr=80.
\end{equation}
A sketch of $u$ is depicted in Figure~\ref{fig:exact_u_3}, for the case $\parr=10$. We consider the same diffusivity tensor as for Test~1, i.e. $\Kmatr=\Kmatr_1$, and then we compare the convergence history obtained by considering \textit{dofi--dofi}, \textit{D--recipe} and RB stabilization with $M=1$. In this test, for the reduced basis stabilization, we plot only on the case $M=1$, since for larger values of $M$, analogously to what happens in the previous case, no significant improvement can be observed. The results are shown in Figure~\ref{fig:stab_test_3} and Table~\ref{tab:errors_test3}: as already observed in the previous test case, the results obtained by RB stabilization improve the performance of the method with respect to standard \textit{dofi--dofi} and \textit{D--recipe} stabilizations. %for both $\erruno{\PiNabla u_h}$ and $\erren{\PiNabla u_h}$.

\begin{figure}%[h!]
	\centering
	\includegraphics[width=0.45\linewidth]{figures/stabilization/test_s_plot}
	\includegraphics[width=0.45\linewidth]{figures/stabilization/test_s_cont}
	\caption{Surface plot and contour plot for the exact solution $u$ defined in \eqref{eq:sol_test_3}. In this case, we set $\parr=10$.}
	\label{fig:exact_u_3}
\end{figure}

\begin{figure}%[h!]
	\centering
	\textbf{Comparison of stabilization terms - Test 2}
	\subfloat{\includegraphics[width=0.43\linewidth]{figures/stabilization/test_s_h1}}
	\subfloat{\includegraphics[width=0.44\linewidth]{figures/stabilization/test_s_en}}
	\caption{Convergence plots for Test 2. Same format of Figure~\ref{fig:stab_test_1}. The reduced basis stabilization improves the results of \textit{dofi--dofi} and \textit{D--recipe} in terms of $\erruno{\PiNabla u_h}$ and $\erren{\PiNabla u_h}$.}
	\label{fig:stab_test_3}
\end{figure}

\renewcommand{\arraystretch}{1.4}
\begin{table}
	\begin{center}
		\begin{tabular}{c||rr|rr||rr|rr}
			%\hline
			\multicolumn{9}{c}{\textbf{Test 2 - Convergence history}}\\
			\hline
			& \multicolumn{4}{c||}{\em dofi--dofi} & \multicolumn{4}{c}{Reduced Basis, $M=1$} \\
			\hline
			$h$ & $\erruno{\PiNabla u_h}$ & Rate & $\erren{\PiNabla u_h}$ & Rate & $\erruno{\PiNabla u_h}$ & Rate & $\erren{\PiNabla u_h}$ & Rate  \\
			\hline
			3.021e-2	& 9.966e-1	& --	& 9.991e-1	& --	& 9.935e-1	& --	& 9.971e-1	& -- \\
			1.536e-2	& 9.979e-1	& 0.02	& 9.714e-1	& 0.04	& 9.596e-1	& 0.05	& 9.486e-1	& 0.07 \\
			7.569e-3	& 9.189e-1	& 0.09	& 8.959e-1	& 0.11	& 8.469e-1	& 0.17	& 8.192e-1	& 0.20 \\
			5.548e-3	& 8.502e-1	& 0.25	& 8.209e-1	& 0.28	& 7.356e-1	& 0.45	& 7.041e-1	& 0.48 \\
			4.094e-3	& 7.416e-1	& 0.44	& 7.202e-1	& 0.43	& 5.851e-1	& 0.75	& 5.799e-1	& 0.63 \\
			3.219e-3	& 5.961e-1	& 0.90	& 5.699e-1	& 0.97	& 4.200e-1	& 1.37	& 4.021e-1	& 1.52 \\
			2.063e-3	& 4.301e-1	& 0.73	& 4.150e-1	& 0.71	& 2.703e-1	& 0.99	& 2.653e-1	& 0.93 \\
			\hline
		\end{tabular}
	\end{center}
	\caption{Errors and convergence rates for Test 2. We focus on VEM with \emph{dofi--dofi} stabilization and reduced basis stabilization with $M=1$.}
	\label{tab:errors_test3}
\end{table}
\renewcommand{\arraystretch}{1}

}


\subsubsection*{Test 3.} For this test, the right hand side is defined according to the following solution and matrix $\Kmatr$. We choose a solution with discontinuous gradient when $x=1/2$. More precisely, $u$ is the continuous piecewise function % \rosso{[Test 6 della cartella dei risultati]}
\begin{equation}\label{eq:sol_test_2}
u(x,y) = \begin{cases}
	\sin(2\pi x)\sin(\paru\pi y)\cos(\pi x) & x\leq \frac{1}{2} \\
	\cos(\paru\pi x) \cos(\pi x) \sin(\paruu(\pi-y)\pi) & x > \frac{1}{2} \\
\end{cases},\qquad \paru=80,\,\paruu=30.
\end{equation}
As shown in Figure~\ref{fig:exact_u_2} for the simplified case with $\paru=10,\,\paruu=15$, this function oscillates in $y$ direction for $0\le x \le 1/2$ and in both $x$ and $y$ directions for $1/2 < x \le 1$. \rev{Then, we set $\Kmatr=\Kmatr_2$, which is a nonsymmetric positive definite matrix.} %Then, we choose the following nonsymmetric positive definite matrix
%\begin{equation*}
%	\Kmatr = \begin{bmatrix}
%		1 & 10^{-2} \\
%		5\cdot10^{-3} & 10^{-4}
%	\end{bmatrix}.
%\end{equation*}
The results  are collected in Figure~\ref{fig:stab_test_2} and Table~\ref{tab:errors_test2} and are mostly in line with the results of the previous tests. Once again, the method with reduced basis stabilization (with $M=1$) performs better than standard cases when $\erruno{\PiNabla u_h}$ is analyzed. Conversely, if we look at $\erren{\PiNabla u_h}$, all the method have same behavior until the last two finest cases, where the use of the reduced basis approach slightly improves.


\begin{figure}%[h!]
\centering
\includegraphics[width=0.45\linewidth]{figures/stabilization/test2_plot}
\includegraphics[width=0.45\linewidth]{figures/stabilization/test2_cont}
\caption{Surface plot and contour plot for the exact solution $u$ defined in \eqref{eq:sol_test_2}. In this case, we set $\paru=10$ and $\paruu=15$.}
\label{fig:exact_u_2}
\end{figure}

\begin{figure}%[h!]
\centering
\textbf{Comparison of stabilization terms - Test 3}
\subfloat{\includegraphics[width=0.43\linewidth]{figures/stabilization/test_2_h1}}
\subfloat{\includegraphics[width=0.44\linewidth]{figures/stabilization/test_2_en}}
\caption{Convergence plots for Test 3. Same format of Figure~\ref{fig:stab_test_1}. Also in this test it is evident that the reduced basis stabilization improves the results of \textit{dofi--dofi} and \textit{D--recipe} in terms of $\erruno{\PiNabla u_h}$. Conversely, all the approaches behave similarly when $\erren{\PiNabla u_h}$ is considered.}
\label{fig:stab_test_2}
\end{figure}

\renewcommand{\arraystretch}{1.4}
\begin{table}
\begin{center}
	\begin{tabular}{c||rr|rr||rr|rr}
		%\hline
		\multicolumn{9}{c}{\textbf{Test 3 - Convergence history}}\\
		\hline
		& \multicolumn{4}{c||}{\em dofi--dofi} & \multicolumn{4}{c}{Reduced Basis, $M=1$} \\
		\hline
		$h$ & $\erruno{\PiNabla u_h}$ & Rate & $\erren{\PiNabla u_h}$ & Rate & $\erruno{\PiNabla u_h}$ & Rate & $\erren{\PiNabla u_h}$ & Rate  \\
		\hline
		3.021e-2	& 9.077e-1	& --	& 7.833e-1	& --	& 9.255e-1	& --	& 7.787e-1	& -- \\
		1.536e-2	& 7.589e-1	& 0.26	& 4.595e-1	& 0.79	& 7.576e-1	& 0.30	& 4.584e-1	& 0.78 \\
		7.569e-3	& 6.736e-1	& 0.17	& 2.522e-1	& 0.85	& 6.468e-1	& 0.22	& 2.501e-1	& 0.85 \\
		5.548e-3	& 6.327e-1	& 0.20	& 1.893e-1	& 0.93	& 5.842e-1	& 0.33	& 1.853e-1	& 0.97 \\
		4.094e-3	& 5.779e-1	& 0.30	& 1.443e-1	& 0.89	& 5.049e-1	& 0.48	& 1.377e-1	& 0.98 \\
		3.219e-3	& 5.062e-1	& 0.55	& 1.108e-1	& 1.09	& 4.133e-1	& 0.83	& 1.019e-1	& 1.25 \\
		2.063e-3	& 4.165e-1	& 0.44	& 8.364e-2	& 0.63	& 3.148e-1	& 0.61	& 7.360e-2	& 0.73 \\
		\hline
	\end{tabular}
\end{center}
\caption{Errors and convergence rates for Test 3. We focus on VEM with \emph{dofi--dofi} stabilization and reduced basis stabilization with $M=1$.}
\label{tab:errors_test2}
\end{table}
\renewcommand{\arraystretch}{1}


\newcommand{\vemglobRB}{V_h^{\text{rb}}}
\newcommand{\vemlocRB}{V^{\text{rb}}}
\newcommand{\nK}{\nu^K}
\newcommand{\Blocort}{\mathbb{B}^\perp(\bK)}







\begin{remark}
It is interesting to observe that the method resulting from the RB stabilization with $M$ basis functions can be interpreted as a fully conforming method in a suitable discretization space~$\vemglobRB$. Indeed, letting $\Blocort$ be defined as
\[
\Blocort = \{ v \in H^{1/2}(\bK) : \quad \int_{\bK} v \nabla q \cdot \nK \,ds= 0, \ \forall q \in \mathbb{P}_1(K), \ \int_{\bK} v\,ds = 0\}, 
\]
we have that $\PiNabla v = 0$ if and only if $v \in \Blocort$.
We can now let $W^\text{rb}(K) \subseteq H^1(K)$ be defined as
\[
W^{\text{rb}}(K) = \{ v \in \Span\{e_1^\text{rb},\cdots,e_N^{\text{rb}}\} :  
v|_{\bK} \in \Blocort
\},
\]
and let 
\[
\vemlocRB(K) = \mathbb{P}_1(K) \oplus W^{\text{rb}}(K).
\] 
Remark that we have that $\mathbb{P}_1(K) \subseteq 	\vemlocRB(K)$ by construction and that ${\vemlocRB}_{|\bK} = \Bkloc$. Thanks to~\eqref{splitting:2}, it is not difficult to check that, if we define
\[
\vemglobRB = \{v \in V : v_{|K} \in \vemlocRB(K)\ \text{ for all }K \in \mesh\},
\]
and we discretize Problem \ref{pro:cont_poisson} by a conforming Galerkin method, we obtain the same linear system as for the VEM method with RB stabilization.
\end{remark}

\section{Application II: Post-Processing}\label{sec:postproc}
Another possible use for the RB reconstruction of virtual element functions is the design of a post-processing technique where the whole $u_h$ is reconstructed, allowing, in particular, to retrieve a conformal approximation to the true solution out of the virtual element degrees of freedom. This can be used for visualization, for evaluating point values, or, for academic purpose, to compute the actual $H^ 1(\Omega)$ error with respect to a known benchmark solution. Also here the idea is to use the RB reconstruction on the non polynomial part of the solution, while evaluating the polynomial part by the standard VEM approach. 

\input{algorithm_postproc}


We demonstrate this approach on three examples where we solve Problem~\ref{pro:basis1} with $\Kmatr=I$ on \rev{$\Omega=(0,1)^2$}, once again discretized by Voronoi meshes. 

In the first example, once the equation is solved with VEM with {\em dofi-dofi} stabilization, we use the reduced basis method to reconstruct the solution and visualize it. In the second example we use the RB reconstruction for evaluating the solution along a line. The third example is an academic convergence test, where the true solution is known and the discrete solution is reconstructed element by element in the entire $\Omega$ to compare the convergence of the post-processed solution $\uhRB$ with the standard $\PiNabla u_h$ and the ``exact" reconstruction $u^\text{fe}_h$.

\subsubsection*{Visualization}

For this test, we discretize $\Omega$ with a relatively coarse Voronoi mesh $\mesh$ consisting of 100 elements, as represented in Figure~\ref{fig:mesh_rec}. For visualization purposes, we solve the Poisson problem by means of the standard lowest order virtual element method and then we recostruct a conforming solution via RB method. The right hand side $f$ is chosen in such a way that the continuous solution is 
\begin{equation}\label{eq:sol_post}
u(x,y) = \frac{1}{32\pi^2} \sin(4\pi x)\sin(4\pi y).
\end{equation}

In Figure~\ref{fig:comparison_postproc}, we plot the reduced basis reconstruction $\uhRB$ (computed in each element of $\mesh$ with precision $M=1$) and we compare it with the standard polynomial projection $\PiNabla u_h$. The reduced basis reconstruction is conforming in the VEM space, while $\PiNabla u_h$ is discontinuous across the elements.%, since the projection operator is defined locally.


%In Figure~\ref{fig:comparison_postproc}, we plot the exact solution $u$, the post-processed solution with projection $\PiNabla u_h$ and the reduced basis reconstruction $\uhRB,\,M=1$ on the mesh represented in Figure~\ref{fig:mesh_rec}, which is part of $\meshfamily$. We then compare the results by analyzing the relative errors $\errzero{\diamond},\erruno{\diamond}$ and $\errinf{\diamond}$. From Figure~\ref{fig:convergence}, it is clear that the reduced basis approximation (orange line) presents the same properties of $u_h$ (black line), slightly improving the behavior of $\PiNabla u_h$ (blue line). Looking at $\errinf{\diamond}$, we see that the good behavior of $\uhRB$ is confirmed also pointwise, as already observed when we carried out the reconstruction in subdomain.

\begin{figure}%[h!]
\centering
%\textbf{Comparison of post processing techniques}\par\medskip
\subfloat[$u$]{\includegraphics[width=0.32\linewidth]{figures/postproc_an}}
\subfloat[$\PiNabla u_h$]{\includegraphics[width=0.32\linewidth]{figures/postproc_pi}}
\subfloat[$\uhRB,\,M=1$]{\includegraphics[width=0.32\linewidth]{figures/postproc_rb1}}
\caption{From left to right: the exact solution $u$ defined in \eqref{eq:sol_post}, the post-processed solution $\PiNabla u_h$ computed projecting onto polynomials in each element, the reconstructed solution $\uhRB$, computed with a single reduced basis in each element. The considered mesh is represented in Figure~\ref{fig:mesh_rec}.}
\label{fig:comparison_postproc}
\end{figure}


\subsubsection*{Local reconstruction}
In this second post-processing example, we solve again the problem under consideration on the mesh depicted in Figure~\ref{fig:mesh_rec}. The right hand side is chosen in such a way that the continuous solution is 
\begin{equation}
\begin{aligned}
	u(x,y) =\,&x^3-xy^2+yx^2+x^2-xy\\
	&\quad -x+y-1+\sin(5x)\sin(7y)+\log(1+x^2+y^4).
\end{aligned}
\end{equation}

Once the degrees of freedom of the discrete solution are computed, the function is reconstructed on the diagonal $y=x$ of the domain, which is marked in red in Figure~\ref{fig:mesh_rec}. We reconstruct the VEM basis functions in each polygon $\elementVEM$ intersecting the diagonal and then we evaluate the solution on a one dimensional grid. For the explicit finite elements computation of the virtual functions in $\elementVEM$, we generate a triangulation $\meshK$ with size $\dd = h_\elementVEM/100$, while the reduced basis reconstruction $\uhRB$ is computed for $M=1,3$.

%We plot the post processed solutions in Figure~\ref{fig:reconstructions}: we represent in black the ``exact" reconstruction $u_h$, in \#\# the reduced basis reconstruction $\uhRB$ and in \#\# the projection $\PiNabla u_h$. It is clear that both $\uhRB$ and $\PiNabla u_h$ give admissible results accordingly to the theory. Of course, the reduced basis reconstruction is conforming in the VEM space, while $\PiNabla u_h$ is discontinuous across the elements, since the operator $\PiNabla$ is defined locally. 

We plot the post-processed solutions in Figure~\ref{fig:reconstructions}. In particular, in Figure~\ref{fig:rec_rb} we compare $\uhRB$ built using $M=3$ (magenta) with $u^\text{fe}_h$ (black), whereas in Figure~\ref{fig:rec_pi} we compare $\PiNabla u_h$ (blue) with $u^\text{fe}_h$. Finally, in Figure~\ref{fig:rec_zoom}, we zoom in the interval $[0.4,0.6]$ to highlight the different behaviors between the reconstructed solutions, considering also $\uhRB,M=1$ (green). \rosso{As already observed in the previous test, both $\uhRB$ and $\PiNabla u_h$ are good approximations of the solution: $\uhRB$ is conforming in the VEM space, whereas $\PiNabla u_h$ is discontinuous.}%In terms of comparison between post processing techniques, the results are in line with the previous test. Concerning the reduced basis reconstruction, looking in particular at Figure~\ref{fig:rec_zoom}, we notice that $\uhRB,\,M=1$ is globally good, but it does not coincide with $u^\text{fe}_h$, as happens when $M=3$ is considered. However, this is a negligible error: in the next example, we will see that the pointwise convergence curve of $\uhRB,\,M=1$ coincides with that of the exact reconstruction $u^\text{fe}_h$.

%	\begin{figure}%[h!]
%		\centering
%		\includegraphics[width=0.5\linewidth]{figures/reconstruction/mesh}
%		\caption{\rosso{DA RISCRIVERE.} Voronoi mesh for the unit square used in the reconstruction test. We highlight in yellow the elements containing the evaluation points we choose on the diagonal.}
%		\label{fig:mesh_rec}
%	\end{figure}
%	
%	\begin{figure}%[h!]
%		\centering
%		\textbf{Reconstruction in subdomain}
%		\subfloat[$\uhRB$ vs $u_h$]{\includegraphics[width=0.35\linewidth]{figures/reconstruction/rbasis3}}
%		\subfloat[$\PiNabla u_h$ vs $u_h$]{\includegraphics[width=0.359\linewidth]{figures/reconstruction/projected}}
%		\subfloat[Comparison]{\includegraphics[width=0.359\linewidth]{figures/reconstruction/zoom}}
%		\caption{\rosso{DA RISCRIVERE.} Comparison of reconstructed functions on $y=x$ of the unit square. The black line represents the exact reconstruction $u_h$, while the magenta line represents the reduced basis approximation with three functions. We plot in blue the piecewise discontinuous $\PiNabla u_h$.}
%		\label{fig:reconstructions}
%	\end{figure}

\begin{figure}
\centering
\textbf{Local reconstruction test}
\subfloat[Geometry \label{fig:mesh_rec}]{\includegraphics[width=0.4\linewidth]{figures/reconstruction/mesh}}
\subfloat[$\uhRB$ vs $u^\text{fe}_h$ \label{fig:rec_rb}]{\includegraphics[width=0.45\linewidth]{figures/reconstruction/rbasis3}}\\
\subfloat[$\PiNabla u_h$ vs $u^\text{fe}_h$ \label{fig:rec_pi}]{\includegraphics[width=0.45\linewidth]{figures/reconstruction/projected}}
\subfloat[Zoom \label{fig:rec_zoom}]{\includegraphics[width=0.45\linewidth]{figures/reconstruction/zoom}}
\caption{Geometry and results for the local reconstruction test. \textsc{(a)}~The problem is solved on a Voronoi mesh and the solution is reconstructed on the red diagonal. \textsc{(b)}~Comparison between the ``exact" reconstruction $u^\text{fe}_h$ (black line) and the reduced basis approximation $\uhRB,M=3$ (magenta line). \textsc{(c)}~Comparison between $u^\text{fe}_h$ and the projection $\PiNabla u_h$ (blue line). \textsc{(d)}~Zoom in the interval $[0.4,0.6]$ comparing $u^\text{fe}_h$, $\PiNabla u_h$, $\uhRB,M=3$ and in addition $\uhRB,M=1$ (green line). All the reconstructions are globally good: $\uhRB,M=1,3$ are conforming, while $\PiNabla u_h$ is discontinuous across the elements.}
\label{fig:reconstructions}
\end{figure}


\subsubsection*{Convergence test}

In this example, the reduced basis post-processing technique is analyzed in terms of convergence properties. We solve the Poisson problem on a sequence of Voronoi meshes $\meshfamily$. We select the exact solution \eqref{eq:sol_post} already chosen for the visualization test.

Once the problem is solved with VEM, we compute the reduced basis reconstruction $\uhRB$ with $M=1$ and we compare its convergence history with those given by the polynomial projection $\PiNabla u_h$ and the ``exact" reconstruction $u^\text{fe}_h$, constructed as in the previous section.

The results are studied in terms of $\errzero{\diamond},\erruno{\diamond},\errinf{\diamond}$ and the convergence plots are collected in Figure~\ref{fig:convergence}. It is clear that the reduced basis approximation (orange line) presents the same convergence history of $u^\text{fe}_h$ (black line), slightly improving the behavior of $\PiNabla u_h$ (blue line). Looking at $\errinf{\diamond}$, we see that the good behavior of $\uhRB$ is confirmed also pointwise, as already observed in the previous test when we carried out a local reconstruction.

\begin{figure}%[h!]
\centering
\textbf{Comparison of post-processing techniques}\par\medskip
\includegraphics[width=0.48\linewidth]{figures/err_l2}
\includegraphics[width=0.485\linewidth]{figures/err_h1}
\includegraphics[width=0.48\linewidth]{figures/err_linf}
\caption{Convergence plots comparing the error committed by $\PiNabla u_h$ (blue line), the ``exact'' reconstruction $u^\text{fe}_h$ (black line) and the reduced basis approximation $\uhRB$ (orange line) computed with a single basis. The reduced basis approximation behaves like $u^\text{fe}_h$ for all the considered errors.}
\label{fig:convergence}
\end{figure}

